JumpCoder: Go Beyond Autoregressive Coder via Online Modification

While existing code large language models (code LLMs) exhibit impressive capabilities in code generation, their autoregressive sequential generation inherently lacks reversibility. This limitation hinders them from timely correcting previous missing statements during coding as humans do, often leading to error propagation and suboptimal performance. We introduce JumpCoder, a novel model-agnostic framework that enables human-like online modification and non-sequential generation to augment code LLMs. The key idea behind JumpCoder is to insert new code into the currently generated code when necessary during generation, which is achieved through an auxiliary infilling model that works in tandem with the code LLM. Since identifying the best infill position beforehand is intractable, we adopt an \textit{infill-first, judge-later} strategy, which experiments with filling at the $k$ most critical positions following the generation of each line, and uses an Abstract Syntax Tree (AST) parser alongside the Generation Model Scoring to effectively judge the validity of each potential infill. Extensive experiments using six state-of-the-art code LLMs across multiple and multilingual benchmarks consistently indicate significant improvements over all baselines. Our code is public at https://github.com/Keytoyze/JumpCoder.

==> table/baseline.tex <==
\begin{table*}[t!]
\centering
\small
\caption{(Full results of \cref{fig:baselines}) The comparative analysis of \model~against various baselines. $^\#$: Disable the generation model to output \texttt{\#} and \texttt{pass} for removing invalid placeholder programs.}
\label{tab:baseline}
% \resizebox{\linewidth}{!}{

\begin{scriptsize}
\begin{tabular}{lrcccc}
\toprule
\multirow{2}[4]{*}{\textbf{Generation model}} & \multirow{2}[4]{*}{\textbf{Size}} & \multirow{2}[4]{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Setting}} \\
\cmidrule{4-6}     &      &      & Vanilla & Filtered & Oracle \\
\midrule
     \multirow{14}[2]{*}{\textsc{CodeLlama-Instruct}} & \multirow{14}[2]{*}{7B} & \method{Greedy-Decoding} & 36.0 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & \textbf{41.5} & - \\
     &      & \method{Self-Infilling} $(N=0)$ & 31.7    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$ & 36.0    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$ & 27.4   & -  & - \\
     &      & \method{Self-Correct} & 36.0 & 36.0 & 37.2 \\
     &      & \model & 37.8 & 39.6 & 39.6 \\
\arrayrulecolor{gray!80}
\cmidrule{3-6}
\arrayrulecolor{black}
     &      & \method{Greedy-Decoding}$^\#$ & 37.8 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$$^\#$ & -    & \textbf{41.5} & - \\
     &      & \method{Self-Infilling} $(N=0)$$^\#$ & 32.9    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$$^\#$ & 37.8    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$$^\#$ & 29.3   & -  & - \\
     &      & \method{Self-Correct}$^\#$ & 37.2 & 37.2 & 39.0 \\
     &      & \model$^\#$ & \textbf{40.2} & \textbf{41.5} & \textbf{41.5} \\
    \midrule

     \multirow{8}[2]{*}{\textsc{CodeLlama-Python}}&   \multirow{8}[2]{*}{7B}    & \method{Greedy-Decoding} & 38.4 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 44.5  & - \\
     &      & \method{Self-Correct} & 40.2  & 40.2  & 40.2 \\
     &      & \model & 40.2 & 41.5 & 41.5 \\
     \arrayrulecolor{gray!80}
\cmidrule{3-6}
\arrayrulecolor{black}
      & & \method{Greedy-Decoding}$^\#$ & 42.7 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$$^\#$ & -    & 43.9  & - \\
     &      & \method{Self-Correct}$^\#$ & 42.1  & 42.1  & 42.7 \\
     &      & \model$^\#$ & \textbf{46.3} & \textbf{46.3} & \textbf{47.6} \\
\midrule

     \multirow{14}[2]{*}{\textsc{CodeLlama-Instruct}}&   \multirow{14}[2]{*}{13B}   & \method{Greedy-Decoding} & 40.9 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 43.3  & - \\
     &      & \method{Self-Infilling} $(N=0)$ & 34.8    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$ & 43.3    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$ & 37.2    & -  & - \\
     &      & \method{Self-Correct} & 41.5 & 41.5 & 41.5  \\
     &      & \model & 44.5 & 43.9 & 45.7 \\
\arrayrulecolor{gray!80}
\cmidrule{3-6}
\arrayrulecolor{black}
      &  & \method{Greedy-Decoding}$^\#$ & 43.9 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$$^\#$ & -    & 43.9  & - \\
     &      & \method{Self-Infilling} $(N=0)$$^\#$ & 37.2    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$$^\#$ & 43.3    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$$^\#$ & 36.0    & -  & - \\
     &      & \method{Self-Correct}$^\#$ & 44.5 & 44.5 & 44.5  \\
     &      & \model$^\#$ & \textbf{45.7} & \textbf{45.7} & \textbf{48.2} \\
\midrule

    \multirow{8}[2]{*}{\textsc{CodeLlama-Python}} &   \multirow{8}[2]{*}{13B}   & \method{Greedy-Decoding} & 43.9 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 48.2  & - \\
     &      & \method{Self-Correct} & 45.1  & 45.1 & 45.7 \\
     &      & \model & 45.7 & 45.7 & 47.0 \\
\arrayrulecolor{gray!80}
\cmidrule{3-6}
\arrayrulecolor{black}
      &  & \method{Greedy-Decoding}$^\#$ & 48.8 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$$^\#$ & -    & 48.8  & - \\
     &      & \method{Self-Correct}$^\#$ & 50.0  & 50.0 & 50.6 \\
     &      & \model$^\#$ & \textbf{50.6} & \textbf{50.6} & \textbf{51.2} \\
\bottomrule
\end{tabular}%
\end{scriptsize}

\end{table*}








==> table/baseline_wo_badwords.tex <==
\begin{table*}[htbp]
\centering
\small
\caption{The comparative analysis of \model~against various baselines, while empty programs are not filtered.}
\label{tab:baseline}
% \resizebox{\linewidth}{!}{


\begin{tabular}{lrcccc}
\toprule
\multirow{2}[4]{*}{\textbf{Generation model}} & \multirow{2}[4]{*}{\textbf{Size}} & \multirow{2}[4]{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Setting}} \\
\cmidrule{4-6}     &      &      & Vanilla & Filtered & Oracle \\
\midrule
\multirow{7}[2]{*}{\textsc{CodeLlama-Instruct}} & \multirow{7}[2]{*}{7B} & \method{Greedy-Decoding} & 36.0 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & \textbf{41.5} & - \\
     &      & \method{Self-Infilling} $(N=0)$ & 31.7    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$ & 36.0    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$ & 27.4   & -  & - \\
     &      & \method{Self-Correct} & 36.0 & 36.0 & 37.2 \\
     &      & \model & \textbf{37.8 (+1.8)} & \textbf{39.6 (+3.6)} & \textbf{39.6 (+3.6)} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{4}[2]{*}{\textsc{CodeLlama-Python}} & \multirow{4}[2]{*}{7B} & \method{Greedy-Decoding} & 38.4 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 44.5  & - \\
     &      & \method{Self-Correct} & 40.2  & 40.2  & 40.2 \\
     &      & \model & \textbf{40.2 (+1.8)} & \textbf{41.5 (+3.1)} & \textbf{41.5 (+3.1)} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{7}[2]{*}{\textsc{CodeLlama-Instruct}} & \multirow{7}[2]{*}{13B} & \method{Greedy-Decoding} & 40.9 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 43.3  & - \\
     &      & \method{Self-Infilling} $(N=0)$ & 34.8    & -  & - \\
     &      & \method{Self-Infilling} $(N=1)$ & 43.3    & -  & - \\
     &      & \method{Self-Infilling} $(N=2)$ & 37.2    & -  & - \\
     &      & \method{Self-Correct} & 41.5 & 41.5 & 41.5  \\
     &      & \model & \textbf{44.5 (+3.6)} & \textbf{43.9 (+3.0)} & \textbf{45.7 (+4.8)} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{4}[2]{*}{\textsc{CodeLlama-Python}} & \multirow{4}[2]{*}{13B} & \method{Greedy-Decoding} & 43.9 & -    & - \\
     &      & \method{Beam-Search} $(S=2)$ & -    & 48.2  & - \\
     &      & \method{Self-Correct} & 45.1  & 45.1 & 45.7 \\
     &      & \model & \textbf{45.7 (+1.8)} & \textbf{45.7 (+1.8)} & \textbf{47.0 (+3.1)} \\
\bottomrule
\end{tabular}%






% }
\end{table*}

==> table/multi.tex <==
\begin{table*}[ht]
\centering
\small
\caption{Results of Pass@1 (\%) on MultiPL-E using greedy generation. V = \underline{V}anilla. O = \underline{O}racle.\\}
\label{tab:multi}
% \resizebox{\linewidth}{!}{

\begin{tabular}{lrcccc}
\toprule
\textbf{Generation model} & \textbf{Size} & \textbf{Method} & \textbf{Python} & \textbf{Java} & \textbf{C++} \\
\midrule
\multirow{3}[2]{*}{\textsc{CodeLlama-Instruct}} & \multirow{3}[2]{*}{7B} & -    & 36.0 & 29.1 & 31.1 \\
     &      & + \model~(V) & \textbf{37.8 (+1.8)} & \textbf{32.3 (+3.2)} & \textbf{34.8 (+3.7)} \\
     &      & + \model~(O) & \textcolor[rgb]{ .502,  .502,  .502}{\textit{39.6 (+3.6)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{33.5 (+4.4)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{36.0 (+4.9)}} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{3}[2]{*}{\textsc{CodeLlama-Python}} & \multirow{3}[2]{*}{7B} & -    & 38.4 & 32.9 & 32.3 \\
     &      & + \model~(V) & \textbf{40.2 (+1.8)} & \textbf{36.7 (+3.8)} & \textbf{34.2 (+1.9)} \\
     &      & + \model~(O) & \textcolor[rgb]{ .502,  .502,  .502}{\textit{41.5 (+3.1)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{39.2 (+6.3)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{34.2 (+1.9)}} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{3}[2]{*}{\textsc{CodeLlama-Instruct}} & \multirow{3}[2]{*}{13B} & -    & 40.9 & 38.6 & \textbf{41.0} \\
     &      & + \model~(V) & \textbf{44.5 (+3.6)} & \textbf{43.0 (+4.4)} & \textbf{41.0 (+0.0)} \\
     &      & + \model~(O) & \textcolor[rgb]{ .502,  .502,  .502}{\textit{45.7 (+4.8)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{44.9 (+6.3)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{42.9 (+1.9)}} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{3}[2]{*}{\textsc{CodeLlama-Python}} & \multirow{3}[2]{*}{13B} & -    & 43.9 & 36.1 & 39.8 \\
     &      & + \model~(V) & \textbf{45.7 (+1.8)} & \textbf{42.4 (+6.3)} & \textbf{42.9 (+3.1)} \\
     &      & + \model~(O) & \textcolor[rgb]{ .502,  .502,  .502}{\textit{47.0 (+3.1)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{44.3 (+8.2)}} & \textcolor[rgb]{ .502,  .502,  .502}{\textit{43.5 (+3.7)}} \\
\arrayrulecolor{gray!80}
\midrule
\arrayrulecolor{black}
\multirow{2}[2]{*}{\# Average} &      & + \model~(V) & (+ 2.3) & (+ 4.4) & (+ 2.2) \\
     &      & + \model~(O) & (+ 3.7) & (+ 6.3) & (+ 3.1) \\
\bottomrule
\end{tabular}%



% }
\end{table*}
